Detection techniques for the H.E.S.S. II telescope, data modeling of gravitational lensing and emission of blazars in HE-VHE astronomy

This thesis presents the study of four aspects of high energy astronomy. The first part of the thesis is dedicated to an aspect of instrument development for imaging atmospheric Cherenkov telescopes, namely the Level 2 trigger system of the High Energy Stereoscopic System (H.E.S.S.). I am providing the motivation and principle of the operation of the Level 2 trigger, I am describing hardware implementation of the system and then I am evaluating expected performances. The second part of my thesis deals with the data analysis and modeling of broad-band emission of particular blazar PKS 1510-089. I am presenting the analysis of the H.E.S.S. data, together with the FERMI data and a collection of multi-wavelength data obtained with various instruments. I am presenting the model of PKS 1510-089 observations carried out during a flare recorded by H.E.S.S.. The third part of my thesis deals with blazars observed by the FERMI-LAT, but from the point of view of other phenomena: a strong gravitational lensing. This part of my thesis shows the first evidence for gravitational lensing phenomena in high energy gamma-rays. This evidence comes from the observation of a gravitational lens system induced echo in the light curve of the distant blazar PKS 1830-211. The last part concentrates on another lensing phenomena called femtolensing. The search for femtolensing effects has been used to derive limits on the primordial black holes abundance. I have used gamma-ray bursts with known redshifts detected by the FERMI Gamma-ray Burst Monitor (GBM) to search for the femtolensing effects caused by compact objects.

==> babelbst.tex <==
%% file: rrmacros.tex = Rob Rutten's old standard LaTeX macros
%% last: Aug 31 2011 
%% site: ~/rr/tex/macros
%% note: ### DO NO LONGER convert to rmacros2e.tex with bindip/convertmacros2e
%%       website sstill use these ones (latex2html not latex2e)
%%       no natbib-needing commands as \cite since then websites don't work
%%       these sit in rrmacros2e

%% text markers
\def\@ #1\par{\par \mbox{}\\ \noindent {\small \tt @ #1}\\[1ex]}  %RR to do
\def\revpar{{{\bf \P\ }}}     %% revision change marker
\def\revpar{}                 %% ignore revision change markers
\long\def\rev#1{{{\bf #1}}}   %% revision change boldface
\long\def\rev#1{#1}           %% ignore revision change boldface

%% ADS character defs
\def\amp{\&}

%% ADS journal abbreviations: long and short versions, also in RJR.BIB
\newcount\longrefs
\def\aap{\ifnum\longrefs=1 {Astron.\ Astrophys.}\else 
                           {A\hbox{\rm \&}A}\fi}
\def\aapr{\ifnum\longrefs=1 {Astron.\ Astrophys.\ Rev.}\else 
                            {A\hbox{\rm \&}AR}\fi}
\def\aaps{\ifnum\longrefs=1 {Astron.\ Astrophys.\ Suppl.}\else 
                            {A\hbox{\rm \&}A Suppl.}\fi}
\def\aj{\ifnum\longrefs=1 {Astron.\ J.}\else 
                          {AJ}\fi} 
\def\ao{\ifnum\longrefs=1 {Applied Optics}\else 
                           {Appl.\ Opt.}\fi} 
\def\aspcs{\ifnum\longrefs=1 {Astron.\ Soc.\ Pacific Conf. Series}\else 
                           {ASP Conf.\ Ser.}\fi} 
\def\apj{\ifnum\longrefs=1 {Astrophys.\ J.}\else 
                           {ApJ}\fi} 
\def\apjl{\ifnum\longrefs=1 {Astrophys.\ J. Lett.}\else 
                            {ApJ}\fi} 
\def\aplett{\ifnum\longrefs=1 {Astrophys.\ J. Lett.}\else 
                            {ApJ}\fi} 
\def\apjs{\ifnum\longrefs=1 {Astrophys.\ J. Suppl.}\else 
                            {ApJS}\fi}
\def\apss{\ifnum\longrefs=1 {Astrophys.\ and Space Science}\else 
                            {Astrophys.\ Space Sci.}\fi}
\def\araa{\ifnum\longrefs=1 {Ann.\ Rev.\ Astron.\ Astrophys.}\else 
                            {ARA\hbox{\rm \&}A}\fi}
\def\azh{\ifnum\longrefs=1 {Astronomicheskii Zhurnal}\else 
                            {Astron.\ Zhur.}\fi}
\def\baas{\ifnum\longrefs=1 {Bull.\ Am.\ Astron.\ Soc.}\else 
                            {BAAS}\fi}
\def\bain{\ifnum\longrefs=1 {Bull.\ Astronom.\ Institutes Netherlands}\else
                            {Bull.\ Astr.\ Inst.\ Neth.}\fi}
\def\gca{\ifnum\longrefs=1 {Geochim.\ Cosmochim.\ Acta}\else 
                           {Geochim.\ Cosmochim.\ Acta}\fi}
\def\grl{\ifnum\longrefs=1 {Geophys.\ Res.\ Lett.}\else 
                           {Geoph.\ Res.\ Lett.}\fi}
\def\iaucirc{\ifnum\longrefs=1 {IAU Circulars}\else 
                          {IAU Circ.}\fi}
\def\ip{\ifnum\longrefs=1 {in press}\else 
                          {in press}\fi}
\def\jgr{\ifnum\longrefs=1 {J.\ Geophys.\ Res.}\else 
                           {J.\ Geophys.\ Res.}\fi}  
\def\jrasc{\ifnum\longrefs=1 {J.\ Royal Astron.\ Soc.\ Canada}\else 
                           {JRAS Can.}\fi}  
\def\memsai{\ifnum\longrefs=1 {Mem.~Soc.~Astron.~Italiana}\else
                              {MemSAI}\fi}
\def\mnras{\ifnum\longrefs=1 {Mon.\ Not.\ Roy.\ Astron.\ Soc.}\else 
                             {MNRAS}\fi} 
\def\nat{\ifnum\longrefs=1 {Nature}\else 
                           {Nat}\fi}
\def\pasj{\ifnum\longrefs=1 {Pub.\ Astron.\ Soc.\ Japan}\else 
                            {PASJ}\fi} 
\def\pasp{\ifnum\longrefs=1 {Pub.\ Astron.\ Soc.\ Pacific}\else 
                            {PASP}\fi} 
\def\physscr{\ifnum\longrefs=1 {Physica Scripta}\else 
                            {Phys.\ Scrip.}\fi} 
\def\planss{\ifnum\longrefs=1 {Planetary \& Space Science}\else 
                            {Plan. \& Space Sci.}\fi} 
\def\prd{\ifnum \longrefs=1 {Physical Review D}\else
                            {Phs.Rev.D}\fi}
\def\prl{\ifnum \longrefs=1 {Physical Review Letter}\else
                            {Phs.Rev.L}\fi}
\def\procspie{\ifnum\longrefs=1 {Proc.\ SPIE}\else 
                            {Proc.\ SPIE}\fi} 
\def\qjras{\ifnum\longrefs=1 {Quarterly J.\ Royal Astron.\ Soc.}\else 
                            {QJRAS}\fi} 
\def\sa{\ifnum\longrefs=1 {Soviet Astron..}\else 
                               {Sov.\ Astron.}\fi}
\def\skytel{\ifnum\longrefs=1 {Sky \& Telescope}\else 
                            {Sky \& Tel.}\fi} 
\def\solphys{\ifnum\longrefs=1 {Solar Phys.}\else 
                               {Sol.\ Phys.}\fi}
\def\ssr{\ifnum\longrefs=1 {Space Science Rev.}\else 
                               {Space\ Sci.\ Rev.}\fi}
\def\zap{\ifnum\longrefs=1 {Zeitschr.\ f.\ Astrophysik}\else
                               {Z.\ Astrophys.}\fi}

%% bibfile specification
\def\bibfiles{/home/rutten/bib/rjrfiles,%
  /home/rutten/bib/rjrfiles}   %% RJR + ADSbibfiles on ~/bib

%% \references (JOURNALS.BIB and AAJOUR.BIB sit in /rrtex/styles)
\def\references{\longrefs=1  \bibliographystyle{rrbib}
             \bibliography{journals,\bibfiles}}
\def\aareferences{\longrefs=0  \bibliographystyle{aabib}
             \bibliography{aajour,\bibfiles}}
\def\apjreferences{\longrefs=0  \bibliographystyle{apjbib}
             \bibliography{aajour,\bibfiles}}
\def\fullreferences{\longrefs=1  \bibliographystyle{namebib}
             \bibliography{journals,\bibfiles}}
\def\fullwwwreferences{\longrefs=1  \bibliographystyle{namewwwbib}
             \bibliography{journals,\bibfiles}}
\def\nlreferences{\longrefs=1  \bibliographystyle{nlbib}
             \bibliography{journals,\bibfiles}}
\def\titlereferences{\longrefs=1  \bibliographystyle{titlebib}
             \bibliography{journals,\bibfiles}}
\def\esareferences{\longrefs=1  \bibliographystyle{esabib} 
             \bibliography{journals,\bibfiles}}
\def\kluwreferences{\longrefs=1 \bibliographystyle{kluwbib}
             \bibliography{journals,\bibfiles}}
\def\kluwtitlereferences{\longrefs=1 \bibliographystyle{kluwtbib}
             \bibliography{journals,\bibfiles}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% link to ADS abstract (use in \href)
\def\linkadscode#1{http://adsabs.harvard.edu/abs/#1}
\def\hrefadscode#1{\href{\linkadscode{#1}}{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  OLD BIBTEX EXPLANATION
%% See AAPAPER.TPL, APJPAPER.TPL, etc in directory tex/templates
%% My RJR-typed -.BIB files are in tex/bibfiles/rjr/bib.
%% My ADS-copied -.BIB files are in tex/bibfiles/ads/bib.
%% Journal abbreviations are specified in AAJOUR.BIB (A&A, APJ format) and
%%   in JOURNALS.BIB (classical longer format), both in tex/styles.
%% The ADS abbreviations are redefined below (in two formats).
%% To use bibtex use script rrbibtex (in ~rutten/rr/bin).
%% Classic cites:
%%          \cite*{Rutten1990a}                        }      
%%               ==>  Rutten (1990)                    } for in-text
%%          \cite*{Gurtovenko+Kostik+Rutten1990b}      } references
%%               ==>  Gurtovenko et al. (1990)        }
%%          \cite{Rutten1990a}                       }
%%               ==>  Rutten 1990                    } for between (...)
%%          \cite{Gurtovenko+Kostik+Rutten1990b}     } references
%%               ==>  Gurtovenko et al. 1990          }
%%          (Rutten 1990a, 1990b)
%%                    \nocite{Rutten1990c}  
%%                    \nocite{Rutten1990f}
%%          NB: \nocite*{..} makes Bibtex produce ALL bibliography entries
%%          NB: Bibtex may mix up the order, putting a later paper
%%              before an earlier one even in the same journal, becauses it
%%              alphabetizes on title after authors.  If it bothers you
%%              then correct the final -.BBL file, or fix the problem
%%              by adding fake digits to TITLE fields in .BIB files. 
%%
%% Full citations for publication lists and PRINTBIB:
%%              \fullreferences (adds full titles and end pages)
%% 
%% References:
%%          - RRBIB: \section*{References} \references 
%%          - FULLBIB: \section*{References} \fullreferences
%%          - AABIB: no section header, \aareferences
%%          - APJBIB: no section header, \apjreferences
%%          - ESA: no BIB.STY, section header ESAPROC.TPL, \esareferences
%%          - set \parsep=0ex to delete blank lines between references
%%          - execute latex, rrbibtex, latex twice
%%          - for email/ftp transfer: comment \references statement out and
%%            merge the -.BBL file there instead, or ftp that as well.
%%            Also ftp or insert this macro file, and email/ftp xxxBIB.STY.
%%
%% Database printout: ps files under /rrtex/bibfiles
%%
%% ADS: As of July 1996 I use ADS entries.  I  pull XXX.BIB files over
%%      from ADS and also XXX.ABS files with the corresponding abstracts.  
%%      They sit in /rrtex/bibfiles/ads/bib and /rrtex/bibfiles/ads/abs.
%%      Script RRBIBTEX copies all the XXX.BIB files to a 
%%      file ~/bib/adsfiles.bib that is searched by BibTeX 
%%      (appropriate BibTeX path in my .login) from script RRBIBTEX.
%%      BibTeX may complain about repeated ADS entries; don't bother.
%% NB: don't refer to the same paper with both its ADS XXX.BIB label 
%%     and its old bibfile label - or you get that reference twice.
%%     Check the resulting reference list for such duplicates.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% INSTITUTE ADDRESS ABBREVIATIONS
\def\nl{,\ } %%\def\nl{\newline}  %% redefine as \newline for mail addresses
\def\AFGL{Air Force Geophysics Lab.\nl Sunspot NM~88349\nl USA}
\def\Arcetri{Osservatorio Astrofisico di Arcetri\nl Largo E. Fermi 5\nl
         I--50125 Firenze\nl Italy}
\def\Armagh{Armagh Observatory\nl College Hill\nl Armagh, BT61~9DG\nl
         Northern Ireland}
\def\ASTRON{Stichting ASTRON\nl Postbus 2\nl NL--7990~AA Dwingeloo\nl
         The Netherlands}
\def\Caltech{Solar Astronomy\nl 105--24 Caltech\nl 
         Pasadena, CA~91125\nl USA}
\def\Catania{Osservatorio Astrofisico di Catania\nl Viale A. Doria 6\nl 
         Citta Universitaria\nl I--95125 Catania\nl Italy}
\def\CfA{Center for Astrophysics\nl 60 Garden Street\nl 
         Cambridge, MA~02138\nl USA}
\def\CHEAF{CHEAF\nl Kruislaan 403\nl NL--1098~SJ Amsterdam}
\def\DAMTP{Dept.\ Applied Math.\ and Theor.\ Phys.\nl Silver Street\nl 
         Cambridge CB3~9EW\nl United Kingdom}
\def\CMAO{Center of Mathematics for Applications, University of Oslo\nl
           P.O. Box 1053, Blindern\nl N-0316 Oslo\nl Norway}
\def\Dwingeloo{Radio Sterrewacht Dwingeloo\nl Postbus 2\nl
      NL--7990 AA Dwingeloo\nl The Netherlands}
\def\ESA{European Space Agency\nl 8--10 Rue Mario Nikis\nl
         F--75738 Paris Cedex 15\nl France} 
\def\ESO{European Southern Observatory\nl Karl--Schwarzschild-Str. 2\nl 
         D--85748 Garching bei M\"unchen\nl Germany}
\def\ESTEC{ESA Space Science Department\nl ESTEC\nl 
         Postbus 299\nl NL--2200~AG Noordwijk\nl The Netherlands}
\def\ETH{Institute of Astronomy\nl ETH--Zentrum\nl 
         CH--8092 Z\"urich\nl Switzerland}
\def\Goddard{NASA Goddard Space Flight Center \nl Greenbelt, MD~20771\nl USA}
\def\Goettingen{Universit\"{a}ts Sternwarte\nl Geismarlandstrasse 11\nl
         D--37083 G\"{o}ttingen\nl Germany}
\def\HAO{High Altitude Observatory\nl NCAR\nl PO Box 3000\nl 
         Boulder, CO 80307--3000\nl USA}
\def\Hawaii{Institute for Astronomy\nl 2680 Woodlawn Drive\nl 
         Honolulu, HAWAII 96822\nl USA}
\def\IAC{Instituto de Astrof{\'{\i}}sica de Canarias\nl C/ Via Lactea S/N\nl
         E--38200 La Laguna, Tenerife\nl Spain}
\def\IAP{Institut d'Astrophysique de Paris\nl 98-bis Boulevard Arago\nl
         F--75014 Paris\nl France}
\def\ISP{Institute for Solar Physics\nl 
         Albanova University Center\nl
         SE--106 91 Stockholm, Sweden}
\def\ITA{Institute of Theoretical Astrophysics\nl
         University of Oslo\nl
         P.O. Box 1029, Blindern\nl N--0315 Oslo\nl Norway}  
\def\JILA{Joint Inst.\ Lab.\ Astrophysics\nl Campus Box 440\nl 
         Univ.\ Colorado\nl Boulder CO 80309--0440\nl USA}
\def\JPL{Jet Propulsion Laboratory\nl 4800 Oak Grove Drive\nl
         Pasadena CA~91109\nl USA}
\def\Kiel{Institut f\"ur Theor.\ Physik und Sternwarte\nl 
         Olshausenstrasse 40\nl D--2300 Kiel 1\nl Germany}  %% postcode?
\def\Kiev{Main Astronomical Observatory\nl Academy of Sciences Ukraine\nl 
         Golosiiv\nl  Kyiv 22\nl  252650 Ukraine}
\def\KIS{Kiepenheuer Institut f\"ur Sonnenphysik\nl Sch\"oneckstrasse 6\nl
         D--79104 Freiburg\nl Germany} 
\def\KSW{Kapteyn Sterrewacht\nl Mensingheweg 20\nl NL--9301 KA Roden\nl
         The Netherlands} 
\def\LKBF{Secretaris/Pennningmeester LKBF\nl \RUL}
\def\LPARL{Lockheed Martin ATC\nl Solar \& Astrophysics Lab\nl 
         Org.\ H1--12, Bldg.\ 252\nl 3251 Hanover Street\nl 
         Palo Alto, CA~94304--1187\nl USA}
\def\Meudon{Observatoire de Paris\nl F--92195 Meudon Principal Cedex\nl 
         France}
\def\NJIT{Department of Physics and Mathematics\nl
          New Jersey Institute of Technology\nl University Heights\nl
          Newark NJ 07102\nl USA}
\def\NOAO{National Opt.\ Astron.\ Obs.\nl P.O. Box 26732\nl 
         Tucson AZ 85726--26732\nl USA}
\def\NRL{Naval Research Laboratory\nl 
         Washington DC 20376--5000\nl USA}   %?? code
\def\NSO{National Solar Observatory\nl PO Box 26732\nl 
         Tucson AZ 85726--6732\nl USA}       
\def\Orsay{Institute d'Astrophysique Spatiale\nl 
         Universit\'e Paris XI--CNRS\nl B\^atiment 121\nl 
         F--91405 Orsay\nl France}
\def\Oslo{Institute of Theoretical Astrophysics\nl
         University of Oslo\nl
         P.O. Box 1029, Blindern\nl N--0315 Oslo\nl Norway}  
\def\OAC{Osservatorio di Capodimonte\nl Via Moiariello 16\nl 
         I--80131 Napoli\nl Italy}
\def\Ondrejov{Astronomical Institute\nl CS--25165 Ondrejov\nl Czech Republic}
\def\Potsdam{Astrophysikalisches Institut\nl Sonnenobservatorium 
         Einsteinturm\nl Telegrafenberg\nl D--14473 Potsdam\nl Germany}
\def\Pulkovo{Pulkovo Observatory\nl Pulskoske Shsee 65--1\nl
         196140 St.\ Petersburg\nl Russia}
\def\RUG{Kapteijn Laboratorium\nl Postbus 800\nl NL--9700~AV Groningen\nl
         The Netherlands}
\def\RUL{Sterrewacht\nl Postbus 9513\nl NL--2300~RA Leiden\nl 
         The Netherlands}
\def\SIU{Sterrekundig Instituut\nl Utrecht University\nl Postbus 80\,000\nl
         NL--3508 TA Utrecht\nl The Netherlands}
\def\SPO{NSO/Sacramento Peak\nl P.O. Box 62\nl 
         Sunspot, NM 88349--0062\nl USA}
\def\Stanford{Center for Space Science and Astrophysics\nl  ERL 328\nl 
         Stanford University\nl Stanford CA 94305--4055\nl  USA}
\def\SRON{SRON\nl Sorbonnelaan 2\nl NL--3584 CA Utrecht\nl The Netherlands}
\def\SRONRUG{SRON\nl Postbus 800\nl NL--9700~AV Groningen\nl 
         The Netherlands}
\def\Uppsala{Astronomiska Observatoriet\nl Box 515\nl S--75120 Uppsala\nl
         Sweden}
\def\UvA{Sterrekundig Instituut ``Anton Pannekoek''\nl Kruislaan 403\nl
         NL--1098~SJ Amsterdam\nl The Netherlands}
\def\VU{Afdeling Sterrekunde\nl Vrije Universiteit\nl De Boelelaan 1081\nl
         NL--1081 HV Amsterdam\nl The Netherlands}
\def\Wuerzburg{Institut f\"ur Astronomie und Astrophysik\nl  Am Hubland\nl
      D--97074 W\"{u}rzburg\nl Germany}

%% blank as long as the given textstring
\newlength{\skipblanklength}
\def\blank#1{\settowidth{\skipblanklength}{#1}\mbox{}\hspace{\skipblanklength}} 
%% no space in this command

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% from DUTCH.STY
\def\dutch{\def\refname{Referenties}\def\abstractname{Samenvatting}%
  \def\bibname{Bibliografie}\def\chaptername{Hoofdstuk}%
  \def\appendixname{Bijlage}\def\contentsname{Inhoudsopgave}%
  \def\listfigurename{Lijst van figuren}%
  \def\listtablename{Lijst van tabellen}%
  \def\indexname{Index}\def\figurename{Figuur}\def\tablename{Tabel}%
  \def\partname{Deel}\def\enclname{Bijlage(n)}\def\ccname{Ter attentie van}%
  \def\headtoname{Aan}\def\headpagename{Pagina}%
  \def\today{\number\day\space\ifcase\month\or januari\or februari\or%
     maart\or%
     april\or mei\or juni\or juli\or augustus\or september\or oktober\or%
     november\or december\fi \space\number\year}}

\hyphenation{Schrij-ver Krij-ger Kuij-pers Bal-le-gooij-en time-slice}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Euro
%% from marvosym.sty
\DeclareFontFamily{OT1}{mvs}{}
\DeclareFontShape{OT1}{mvs}{m}{n}{<-> fmvr8x}{}
\def\mvs{\usefont{OT1}{mvs}{m}{n}}
\def\mvchr{\mvs\char}
\def\textmvs#1{{\mvs #1}}
\def\EUR{{\footnotesize{\mvchr164}}}  %% I don't like standard size
\def\EUR{{\small{\mvchr164}}}  %% I don't like standard size

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% warningoverprint
%% eg: \warningoverprint{DRAFT}, or SUBMITTED, CONFIDENTIAL from Eric Bakker
\def\warningoverprint #1{\special{!userdict begin 
  /bop-hook{gsave 100 600 translate -45 rotate /Times-Roman findfont 
  100 scalefont setfont 0 0 moveto 0.9 setgray (#1) show grestore}def end}}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% figures
%% journal figures, use templettes in AAFIGS.TPL, APJFIGS.TPL, MULTIFIG.TPL
%% mostly obsolete!  maintain for old paper files
\newcounter{onefig} \newcounter{fignumber}
\newcount\nocaptions \newcount\nofigures \newcount\figwidth
\newcount\viewgraphs \newcount\printlabel
\long\def\skipfigure #1\viewout{}   %% use \skipfigure....\viewout
\def\figsfile{} \def\figspath{} \def\paper{} \def\format{} \def\figlabel{} 
\long\def\nextfig#1{\setcounter{figure}{\value{fignumber}}
  \addtocounter{fignumber}{1}
  \ifnum \viewgraphs=1 \pagestyle{empty} \fi 
  \ifnum\value{onefig}=0 #1 \fi                 
  \ifnum\value{onefig}=\value{fignumber} #1 \fi}
\def\figwidths#1#2{\ifnum \nocaptions=1 #2mm \else #1mm \fi}  
\def\picplace{\framebox[80mm]{\rule{0cm}{1cm}}}
\def\paper#1{}  %% redefine for separate-figure identification line
\long\def\plotfig#1#2{\ifnum \nofigures=1 \picplace \else #2 \fi}
\long\def\captiontext#1{\ifnum \nofigures=1 \raggedright \fi 
   \ifnum \nocaptions=1 \paper
     \ifnum \viewgraphs=0 
       \newline  \mbox{}\hrulefill\mbox{} \newline 
       \ifnum \printlabel=1 \{{\em \figlabel}\}\newline \fi
     \fi 
%% \else \ifnum \nofigures=0 \{\figlabel\}~~ \fi   %% adds label
   \else \ifnum \printlabel=1 \{{\em \figlabel}\}\newline \fi
     #1 \fi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MULTI-FILE FIGURE
%% macros to combine separate postscript files into one multi-panel figure;
%% templettes in template files AAFIGS.TPL, APJFIGS.TPL, MULTIFIG.TPL.
%% - measure panel bounding boxes with GHOSTVIEW
%%   - large lower-left (outside axis labels)
%%   - small lower-left (between labels and numbers or just outside frame)
%%   - upper-left
%% - use \barepanel, \labelxpanel, \labelypanel, \labelxypanel 
%%   to control layout, for example to cut all x labels off and replace
%%   by single full-width LaTeX x label.  See templettes or test files.
%%   First specify \panelsize; \panelheight=0 maintains frame aspect ratio.
\newcount\panelwidth \newcount\panelheight 
\newcount\bxmin \newcount\bymin \newcount\bxmax \newcount\bymax
\newcount\tbxmin \newcount\tbymin
\newcount\tpanelwidth \newcount\tpanelheight \newcount\tpdif
\panelwidth=70 \panelheight=70  %% defaults (mm)
\def\panelsize #1,#2;{\panelwidth=#1 \panelheight=#2}  
     %% units MUST be mm
     %% \panelheight=0 or \panelwith=0 maintains frame aspect ratio
\def\setbb #1,#2;#3,#4;#5,#6;{% UNITS: bp (from ghostview)
  \tbxmin=#1 \tbymin=#2    %% full box (axis titles) lower left corner
  \bxmin=#3 \bymin=#4      %% bare box (ticks only) lower left corner
  \bxmax=#5 \bymax=#6}     %% upper right corner
\def\barepanel #1{%
  \ifnum\panelheight=0 
    \tpdif=\bymax \advance\tpdif by -\bymin
    \multiply \tpdif by \panelwidth
    \tpanelheight=\tpdif
    \tpdif=\bxmax \advance\tpdif by -\bxmin
    \divide \tpanelheight by \tpdif
  \else \tpanelheight=\panelheight \fi
  \ifnum\panelwidth=0 
    \tpdif=\bxmax \advance\tpdif by -\bxmin
    \multiply \tpdif by \panelheight
    \tpanelwidth=\tpdif
    \tpdif=\bymax \advance\tpdif by -\bymin
    \divide \tpanelwidth by \tpdif
  \else \tpanelwidth=\panelwidth \fi
  \psfig{figure=#1,%
     bbllx=\bxmin bp,bblly=\bymin bp,bburx=\bxmax bp,bbury=\bymax bp,clip=t,%
     width=\tpanelwidth mm,height=\tpanelheight mm}}
\def\labelypanel #1{% TeX permits only integer arithmetic, so bp and mm
  \ifnum\panelheight=0 
    \tpdif=\bymax \advance\tpdif by -\bymin
    \multiply \tpdif by \panelwidth
    \tpanelheight=\tpdif
    \tpdif=\bxmax \advance\tpdif by -\bxmin
    \divide \tpanelheight by \tpdif
  \else \tpanelheight=\panelheight \fi
  \ifnum\panelwidth=0 
    \tpdif=\bxmax \advance\tpdif by -\bxmin
    \multiply \tpdif by \panelheight
    \tpanelwidth=\tpdif
    \tpdif=\bymax \advance\tpdif by -\bymin
    \divide \tpanelwidth by \tpdif
  \else \tpanelwidth=\panelwidth \fi
  \tpdif=\bxmax \advance\tpdif by -\tbxmin
  \multiply \tpanelwidth by \tpdif
  \tpdif=\bxmax \advance\tpdif by -\bxmin
  \divide \tpanelwidth by \tpdif
  \psfig{figure=#1,%
    bbllx=\tbxmin bp,bblly=\bymin bp,bburx=\bxmax bp,bbury=\bymax bp,%
    clip=t,width=\tpanelwidth mm,height=\tpanelheight mm}}
\def\labelxpanel #1{%
  \ifnum\panelheight=0 
    \tpdif=\bymax \advance\tpdif by -\bymin
    \multiply \tpdif by \panelwidth
    \tpanelheight=\tpdif
    \tpdif=\bxmax \advance\tpdif by -\bxmin
    \divide \tpanelheight by \tpdif
  \else \tpanelheight=\panelheight \fi
  \ifnum\panelwidth=0 
    \tpdif=\bxmax \advance\tpdif by -\bxmin
    \multiply \tpdif by \panelheight
    \tpanelwidth=\tpdif
    \tpdif=\bymax \advance\tpdif by -\bymin
    \divide \tpanelwidth by \tpdif
  \else \tpanelwidth=\panelwidth \fi
  \tpdif=\bymax \advance\tpdif by -\tbymin
  \multiply \tpanelheight by \tpdif
  \tpdif=\bymax \advance\tpdif by -\bymin
  \divide \tpanelheight by \tpdif
  \psfig{figure=#1,%
    bbllx=\bxmin bp,bblly=\tbymin bp,bburx=\bxmax bp,bbury=\bymax bp,%
    clip=t,width=\tpanelwidth mm,height=\tpanelheight mm}}
\def\labelxypanel #1{%
  \ifnum\panelheight=0 
    \tpdif=\bymax \advance\tpdif by -\bymin
    \multiply \tpdif by \panelwidth
    \tpanelheight=\tpdif
    \tpdif=\bxmax \advance\tpdif by -\bxmin
    \divide \tpanelheight by \tpdif
  \else \tpanelheight=\panelheight \fi
  \ifnum\panelwidth=0 
    \tpdif=\bxmax \advance\tpdif by -\bxmin
    \multiply \tpdif by \panelheight
    \tpanelwidth=\tpdif
    \tpdif=\bymax \advance\tpdif by -\bymin
    \divide \tpanelwidth by \tpdif
  \else \tpanelwidth=\panelwidth \fi
  \tpdif=\bxmax \advance\tpdif by -\tbxmin
  \multiply \tpanelwidth by \tpdif
  \tpdif=\bxmax \advance\tpdif by -\bxmin
  \divide \tpanelwidth by \tpdif 
  \tpdif=\bymax \advance\tpdif by -\tbymin 
  \multiply \tpanelheight by \tpdif
  \tpdif=\bymax \advance\tpdif by -\bymin
  \divide \tpanelheight by \tpdif
  \psfig{figure=#1,%
    bbllx=\tbxmin bp,bblly=\tbymin bp,bburx=\bxmax bp,bbury=\bymax bp,%
    clip=t,width=\tpanelwidth mm,height=\tpanelheight mm}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% panel label
%% adds labels to panels, from Louis Strous
%% eg \panellabel{1.5em}{0.5em}{(a)} = 1.5em from right, 0.5em from bottom
\newcommand{\panellabel}[3]{\makebox[0pt][r]{\raisebox{#2} #3 \hspace{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% float params
\def\topfraction{0.99}                      %% to permit many large figures
\def\dbltopfraction{0.99}
\def\textfraction{0.01} 
\def\floatpagefraction{0.99}
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COMMENTS
%% Option for yes/no printing of internal comments within LaTeX output.
%% - Begin comment with new line with %CC 
%% - start each comment line with %, for example with %RR
%% - end comment with new line with %EE and blank line if paragraph end.
%% - example:
%%      %CC
%%      %RR This is a RR comment to his co-authors
%%      %EE
%%
%% For comment printing replace with editor everywhere (after the
%% \begin{document} command):
%%        %CC by \CC 
%%        %EE by \end{verbatim} \EE          
%% and change these back again for skipping comments in LaTeX printout.
%% The other text will be compressed when comments are printed.
%%
%% Skip comments permanently by taking out CC and EE lines. 
%% Don't delete comments if you wish to record evolutionary thinking.  
%%
\def\CC{\par \vspace*{-2ex} \footnotesize \baselineskip=8pt \begin{verbatim}}
\def\EE{\par \vspace*{-2ex} \normalsize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% IGNORE
\long\def\startignore #1\stopignore{}   %% use \startignore....\stopignore

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FULLFIGURE
%% for full-page figure with LaTeX caption use (Mats):
%%      \begin{figure}[p]
%%            \vbox to \textheight{\hbox{}\vfill
%%                  \caption[..]{\it............
%%                               \label{.....}}}
%%      \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TASK
\newenvironment{task}{%
  \begin{list}{$\bullet$}{\itemsep=1ex \parindent=3ex \parskip=1ex 
    \topsep=0ex}}
  {\end{list}}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CAMERA-READY ARTICLE HEADER
%% use for example: 
%%      \begin{koprr}
%%              {\large \bf  TITLE}\\[2ex]
%%              {\bf  AUTHORS}\\[2ex]
%%              {\sl  ADRRESS}\\[3cm]
%%      \end{koprr}
%%
\def\koprr{\list{}{      
  \itemindent=0pt \listparindent=0pt \itemsep=0pt
  \leftmargin=5ex}\item[]}                     %% 5ex = left margin
  \let\endkoprr=\endlist

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FIGURETTE COLUMN
%% Blank column on the right for small figures.  Example: Seattle review
%% See also TeX parshape command and FLOATFIG style
%%
\def\kolom{\list{}{\rightmargin=5cm      %% 5cm = width column at right
  \topsep=0ex \itemsep=0cm \parsep=0ex \parskip=0ex \partopsep=0ex 
  \listparindent=3ex
  \itemindent=0pt \leftmargin=0pt} \item[] 
  \vspace*{-0ex}}                        %% this funny command kills gaps
  \let\endkolom=\endlist

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LIST PARAMETERS
\renewcommand{\labelitemi}{{\bf --}}                %% no bullets but dashes
\def\setlistparams{         
  \topsep=0.7ex                 %% ADAPT: parskip=0: 0.7;  parskip=1: -1.2ex
  \itemsep=0.7ex                %% space between items
  \leftmargini=3ex}             %% dashes at beginning of line 
\setlistparams                  %% recall after type changes 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ALPHABETIC LIST
\newcounter{alistindex}  \newcounter{alistvalue}     %% problems: a)  b) etc
\newenvironment{alist}{%
   \begin{list}{\alph{alistindex})}{\usecounter{alistindex}}
   \itemsep=1ex \parskip=1ex}{\end{list}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LINE SPACING
\def\spacing #1{\small \renewcommand{\baselinestretch}{#1}
                \normalsize \setlistparams}             %% eg: \spacing{1.5}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% UNINDENTED ITEMIZE
%% puts dashes fully left, no extra indent.  As ENUMERR below.
\newenvironment{itemrr}{\vspace*{-\parskip}
  \leftmargini=3ex \topsep=0.6ex       
  \begin{itemize}
     \itemsep=0.5ex \parindent=0ex \parsep=0ex}{
  \end{itemize} \vspace*{-\parskip}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CONDENSED ITEMIZE
%% puts dashes fully left, no extra indent, small top and bottom spacing
%%                                   Example: Solar Physics Newsletter 3
\newenvironment{conditem}{               
  \leftmargini=6ex \topsep=0.2ex 
  \begin{itemize}
     \itemsep=0ex \parindent=3ex \parsep=0ex}{
  \end{itemize}}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% UNINDENTED ENUMERATE
%% puts numbers fully left, no extra indent.  Example: Kiev IAU Summary
\newenvironment{enumerr}{               
  \leftmargini=3ex \topsep=1.5ex       
  \begin{enumerate}
     \itemsep=0.7ex \parindent=3ex \parsep=0ex}{
  \end{enumerate}}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CONDENSED ENUMERATE
%% puts numbers fully left, no extra indent, small top and bottom spacing.
%% Example: Solar Physics Newsletter 2 Huber item
\newenvironment{condenum}{               
  \leftmargini=3ex \topsep=0.5ex 
  \begin{enumerate}
     \itemsep=0ex \parindent=3ex \parsep=0ex}{
  \end{enumerate}}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ROMAN ENUMERATE
%% puts numbers fully left, uses (i), (ii), (iii) etc.                 
\newcounter{romenumnr}
\newenvironment{romanenum}{
  \leftmargini=6ex \topsep=1.5ex
  \begin{list}{(\roman{romenumnr}) --}{\usecounter{romenumnr}
      \itemsep=1ex \listparindent=3ex \parsep=0ex}}{
  \end{list}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% POSTER PAGE
%% one page, shadowframe, large sansserif, for POSTER.TPL
%% usage: \posterpage{header}{text}  
%%        suppress header with {\mbox{}}
%%        text may contain titles, multiple paragraphs, item lists etc.
\newcommand{\posterpage}[2]{{\Large \sf \newpage
  \setlength{\minipagewidth}{\textwidth} \addtolength{\minipagewidth}{-2cm}
  \fboxrule=0.3ex \fboxsep=0ex
  \def\shadowparams{\topsep=-2.5ex \itemsep=-1.5ex \leftmargini=5ex}
  \renewcommand{\labelitemi}{$\bullet$}
  \parskip=3ex \shadowparams
  \savebox{\boxcontent}[\textwidth]{
    \begin{minipage}[t]{\minipagewidth}
        \parskip=3ex \vspace*{1ex}
        \begin{center} \LARGE \bf #1 \end{center} 
        \vspace{2ex} #2 \vspace*{3ex} \mbox{ }
    \end{minipage}}
  \hspace*{\textwidth} \hspace*{-0.8ex} \rule{2ex}{\dp\boxcontent}
  \par \vspace*{-\dp\boxcontent} \vspace*{-7.2ex}
  \framebox[\textwidth]{\usebox{\boxcontent}}
  \par \vspace*{-3.0ex} \hspace*{1.7ex} \rule{\textwidth}{2ex}
  \setlistparams \renewcommand{\labelitemi}{{\bf --}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PDF TALKS
\def\allpdf{/home/rutten/rr/wrt/talks/allpdf}
%% usage: \pdfheader{filename}{title}, eg: \pdfheader{intro}{TALK OUTLINE}
%% upper left: clicks to talk file table; 
%% middle: clicks to talk files table
%% upper right: clicks to pdf dir
\newcommand{\pdfheader}[2]{\hypertarget{#1}{} \sf \parskip=3ex
  \mbox{}\vspace*{-15mm}\par\mbox{} \hspace*{-15mm} 
  \hyperlink{talkstart}{\textcolor{white}
                          {\huge \mbox{talk start}}}
  \hfill
  \hyperlink{setfiletable}{\textcolor{white}
                          {\huge \mbox{~~~~~talk files}}}
  \hfill
  \href{/home/rutten/rr/wrt/talks/pdf/pdfcontents.pdf}
       {\textcolor{white}{\huge \mbox{~~~~~~~all talks}}}
  \par \vspace{1ex}
  \centerline{\Acrobatmenu{GoBack}{\textcolor{Black}{\large #2}}}}

%% usage: \pdfbackheader{filename}{title}: title in orchid, clicks back
%% upper left: clicks to talk file table; upper right: clicks to pdf dir
\newcommand{\pdfbackheader}[2]{\hypertarget{#1}{} 
  \sf \normalsize \parskip=3ex
  \mbox{}\vspace*{-17mm}\par\mbox{} \hspace*{-15mm} 
   \hyperlink{talkstart}{\textcolor{white}
                          {\huge \mbox{talk start}}}
  \hfill
  \hyperlink{setfiletable}{\textcolor{white}
                          {\huge \mbox{~~~~~talk files}}}
  \hfill 
  \href{/home/rutten/rr/wrt/talks/pdf/pdfcontents.pdf}
       {\textcolor{white}{\huge \mbox{~~~~~~~all talks}}}
  \par
  \centerline{\Acrobatmenu{GoBack}{\textcolor{DarkOrchid}{\large #2}}}}

\def\esmnsun{\epsfig{file=/home/rutten/rr/int/ESMN2/logos/esmnlogosun.png,%
           height=17mm}}
\newcommand{\esmnbackheader}[2]{\hypertarget{#1}{} \sf \parskip=3ex
  \mbox{}\vspace*{-12mm}\par\mbox{} \hspace*{-15mm} 
  \hyperlink{setfiletable}{\mbox{~~~~~~~~~~}\esmnsun}
  \hfill 
  \href{/home/rutten/rr/wrt/talks/pdf/pdfcontents.pdf}
       {\esmnsun}
  \par \vspace*{-13mm}
  \centerline{\Acrobatmenu{GoBack}{\textcolor{DarkOrchid}{\LARGE #2}}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% VWGRAPH
%% usage: \vwgraph{width}{header}{text}  
%%        suppress header with: \vwgraph{\mbox{}}{text} 
%%        specify fonts, eg: \vwgraph{\huge \bf ...}{\Large \sf ...}
%%        text may contain titles, paragraphs, item lists etc.
\newcommand{\vwgraph}[3]{\newpage
    \begin{center}
     \shadowframe{#1}{
       \begin{center}
         \vspace*{2ex}
         {\Large \bf #2}\\[4ex]
       \end{center}
       {\Large \sf #3}}   %% ADAPT font
     \end{center}}
\newenvironment{itemvg}{
  \leftmargini=3ex \topsep=0.5ex
  \begin{itemize} \vspace{-1ex}
     \itemsep=0.5ex \parindent=3ex \parsep=0ex}{
  \end{itemize}}
\newenvironment{itemsmall}{
  \leftmargini=3ex \topsep=0.0ex
  \begin{itemize} \vspace{-1.3ex}
     \itemsep=-0.2ex \parindent=3ex \parsep=0ex}{
  \end{itemize}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LECTVW
%% usage: \lectvw{header}{text}  = \vwgraph without shadow box
%%        suppress header with: \vwgraph{\mbox{}}{text} 
%%        specify fonts, eg: \vwgraph{\huge \bf ...}{\Large \sf ...}
%%        text may contain titles, paragraphs, item lists etc.
\long\def\lectvw#1#2{\newpage \vspace*{-15mm}
    \begin{center}
       \begin{center}
         {\LARGE \sc \underline{#1}}\\[4ex]
       \end{center}
       {\Large \sf #2}   %% ADAPT font
     \end{center}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SHADOWFRAME
%% minipage in shadowframe, used in VWGRAPH.TPL 
%% usage: \shadowframe{width}{text}
%%        eg: \shadowframe{15cm}{\large \sf ...}
%%        text may contain titles, paragraphs, item lists etc.
\newlength{\minipagewidth}
\newcommand{\shadowframe}[2]{
  \setlength{\minipagewidth}{#1} \addtolength{\minipagewidth}{-1cm}
  \fboxrule=0.5ex \fboxsep=0ex
  \def\shadowparams{\topsep=-2.5ex \itemsep=-1.5ex \leftmargini=5ex}
  \renewcommand{\labelitemi}{$\bullet$}
  \parskip=3ex \shadowparams 
  \savebox{\boxcontent}[#1]{         
    \begin{minipage}[t]{\minipagewidth}
      \vspace*{1.5ex} #2 \vspace*{0.5ex} \mbox{ } 
    \end{minipage}}
  \hspace*{#1} \hspace*{1.0ex} \rule{2ex}{\dp\boxcontent}  
  \par \vspace*{-\dp\boxcontent} \vspace*{-7.9ex} 
  \framebox[#1]{\usebox{\boxcontent}}  
  \par \vspace*{-3.0ex} \hspace*{4.5ex} \rule{#1}{2ex}
  \setlistparams \renewcommand{\labelitemi}{{\bf --}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OVALHEAD
%% header in centered oval, 3 widths (8cm, 12cm, 16cm), for VWGRAPH.TPL
%% usage: \ovalhead{text}     eg: \ovalhead{\Large \bf Conclusions}
%%        \ovalhead{\mbox{}} suppresses oval
\newsavebox{\boxcontent}
\newcommand{\ovalhead}[1]{
  \unitlength=1cm
  \sbox{\boxcontent}{\mbox{~~{#1}~~}}
  \begin{center}
    \ifdim\wd\boxcontent>6ex 
    \ifdim\wd\boxcontent<8cm 
    \begin{picture}(8,3) \thicklines     
      \put(4.0,0.8){\oval(8,1.6)} 
      \put(0.0,0.7){\parbox{8cm}{
         \begin{center} \usebox{\boxcontent} \end{center}}}
    \end{picture}
    \else \ifdim\wd\boxcontent<12cm 
    \begin{picture}(12,3) \thicklines     
        \put(6.0,0.8){\oval(12,1.6)} 
        \put(0.0,0.7){\parbox{12cm}{
           \begin{center} \usebox{\boxcontent} \end{center}}}
    \end{picture}
    \else
    \begin{picture}(16,3) \thicklines     
        \put(8.0,0.8){\oval(16,1.6)} 
        \put(0.0,0.7){\parbox{16cm}{
           \begin{center} \usebox{\boxcontent} \end{center}}}
    \end{picture}
    \fi \fi \fi
  \end{center}} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COLLOQFRAME
%% shadowed frame, for colloquium and lunch talk announcements
%% use: \colloqframe{width}{text}
\newcommand{\colloqframe}[2]{
  \setlength{\minipagewidth}{#1} \addtolength{\minipagewidth}{-1cm}
  \fboxrule=0.5ex \fboxsep=0ex
  \parskip=3ex
  \savebox{\boxcontent}[#1]{
    \begin{minipage}[t]{\minipagewidth}
      \vspace*{1.5ex} #2 \vspace*{0.5ex} \mbox{ }
    \end{minipage}}
  \hspace*{#1} \hspace*{-0.8ex} \rule{2ex}{\dp\boxcontent}
  \par \vspace*{-\dp\boxcontent} \vspace*{-7.9ex}
  \framebox[#1]{\usebox{\boxcontent}}
  \par \vspace*{-3.0ex} \hspace*{1.7ex} \rule{#1}{2ex}
  \renewcommand{\labelitemi}{{\bf --}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SOL OVAL
%% Old Utrecht sol symbol in label oval for SIU announcement labels 
%% Use: \soloval{text}
\newcommand{\soloval}[1]{\fboxrule=0.5mm \unitlength=1cm
\hspace*{5mm} \sol{20mm}\\[-20mm]
\begin{picture}(15,3) \thicklines
 \put(7.5,2){\oval(15.60,3.60)} \put(7.5,2){\oval(15.55,3.55)}
 \put(7.5,2){\oval(15.50,3.50)} \put(7.5,2){\oval(15.45,3.45)}
 \put(7.5,2){\oval(15.40,3.40)} \put(7.5,2){\oval(15.35,3.35)}
 \put(7.5,2){\oval(15.00,3.00)} \put(2.0,1.9){\parbox{13cm}{#1}}
\end{picture}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SOL
%% new Utrecht sol symbol for letterhead
\def\rrsol#1{%
\epsfig{file=/home/strknd/rutten/rr/tex/templates/rrsol,%
       bbllx=100bp,bblly=570bp,bburx=515bp,bbury=685bp,clip=,%
       width=#1}}
\def\cutsol#1{%
\epsfig{file=/home/strknd/rutten/rr/art/siusol/sol-color,height=#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RR AFFILIATIONS
\def\rruuita{%
  \centerline{Robert J. Rutten}
  \vspace{0.2ex}
  \centerline{Sterrekundig Instituut Utrecht 
              \mbox{~~}\&\mbox{~~}
              Institutt for Teoretisk Astrofysikk Oslo}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SECTION NUMBERING DEPTH
\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{3}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SECTIONRR COMMANDS
                             %% use these for parskip>0 and/or to set labels
\def\chapterrr#1{\chapter{#1} \label{chap:#1} \vskip-\parskip}  
\def\sectionrr#1{\section{#1} \label{sec:#1} \vskip-\parskip}
\def\subsectionrr#1{\subsection{#1} \label{sec:#1} \vskip-\parskip}
\def\subsubsectionrr#1{\subsubsection{#1} \label{sec:#1}  \vskip-\parskip}
\def\paragraphrr#1{\paragraph{#1.} \label{sec:#1} \vskip-\parskip}
                                                     %% #1 without period

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SMALL SECTION HEAD 
\def\smallhead #1{\vspace{2ex} \noindent {\bf #1}~~~\noindent} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ALTERNATIVE SECTION HEADS
%% Alternative section heads
%% Note: often usage of e.g. \subsubsection*{3. Results} is better to
%%       obtain a smaller header since this won't occur at page bottom
\newcounter{headnr}            
\newcounter{subheadnr}[headnr]
\newcounter{subsubheadnr}[subheadnr]
\def\head #1{
  \stepcounter{headnr}                          %% sets subheadnr = 0 too 
  \vspace{3ex} \par \noindent                   %% 2ex = space above, no *
  {\bf \theheadnr~~~~#1}\\[1ex] \noindent}      %% 1ex = space below
\def\subhead #1{  
  \stepcounter{subheadnr}
  \vspace{2ex} \par \noindent
  {\bf \theheadnr.\arabic{subheadnr}~~~#1}\\[1ex] \noindent}
\def\subsubhead #1{
  \stepcounter{subsubheadnr}
  \vspace{1.5ex} \par \noindent
  {\bf \theheadnr.\arabic{subheadnr}.\arabic{subsubheadnr}~~~#1}\\[0.2ex] 
  \noindent}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SPS-EPS NEWSLETTER MACROS 
\def\epstitle #1{\parskip=0ex \vspace{-2ex}
          \subsubsection*{\center \framebox[8.5cm]{\large \bf #1}}
          \parindent=3ex \parskip=0ex}
\def\epsdoubletitle #1#2{\parskip=0ex \vspace{-2ex}
          \subsubsection*{\center {\large \sc #1}}
          \vspace{-0.3ex}
          {\center \framebox[8.5cm]{\large \bf #2}\\[1ex]}
          \parindent=3ex \parskip=0ex \noindent}
\def\epssmalltitle #1{\subsubsection*{
        \vspace{-5ex} \center {\normalsize \sl #1}} \vspace*{-1.0ex}}
\def\epsauthor #1{\par\vspace*{0.3ex} \hspace*{\fill}{\sl#1}\\}
\def\epsinst #1{\hspace*{\fill}{\small#1}\\}
\def\sigrjr{\hspace{1.5cm} \raisebox{-1.5cm}{%
  \epsfig{file=/home/strknd/rutten/rr/adm/letters/figs/rjr,width=4cm}}
       \vspace*{-1.2cm} \par}%
%%     bbllx=75bp,bblly=300bp,bburx=480bp,bbury=500bp,clip=,%
%%     angle=-5,width=4cm}} \vspace*{-1.2cm} \par}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DROPCAP
%%  big "miniature" from DROP.STY from Eric Bakker, use \dropcap{T}he
\font\dropfont= cmr12 scaled \magstep5
\def\dropcap#1#2{{\noindent
    \setbox0\hbox{\dropfont #1}\setbox1\hbox{#2}\setbox2\hbox{(}%
    \count0=\ht0\advance\count0 by\dp0\count1\baselineskip
    \advance\count0 by-\ht1\advance\count0by\ht2
    \dimen1=.5ex\advance\count0by\dimen1\divide\count0 by\count1
    \advance\count0 by1\dimen0\wd0
    \advance\dimen0 by.25em\dimen1=\ht0\advance\dimen1 by-\ht1
    \global\hangindent\dimen0\global\hangafter-\count0
    \hskip-\dimen0\setbox0\hbox to\dimen0{\raise-\dimen1\box0\hss}%
    \dp0=0in\ht0=0in\box0}#2}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% HANGLINE
%% next line indentation.  Usage: \hangline{2ex}.  End last with paragraph
\def\hangline #1{\par\noindent\hangafter=1\hangindent=#1}
%% Jul 17 2010 changed: \parskip=0pt out

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LATIN ABBREVIATIONS
\def\rmit#1{{\it #1}}              %% italics (RR style, Kluwer)
                                   %% redefine for A&A and ApJ, no italics
\def\etal{\rmit{et al.}}           %% use \etal\ for space behind it        
\def\etc{\rmit{etc.}}           
\def\ie{\rmit{i.e.,}}              %% , required (Webster 1681)
\def\eg{\rmit{e.g.,}}              %% , required (Webster 1681)
\def\cf{cf.}                       %% no Latin, always Roman (Webster 1686)
\def\viz{\rmit{viz.}}
\def\vs{\rmit{vs.}}

%%%%%%%%%%%%%%%%%%%%%%%%%% \sofar
\def\sofar{\mbox{}\\[1ex]
  \centerline{\framebox{{\bf @===========   RJR SO FAR   =============}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SPECTRA
\def\specchar#1{\uppercase{#1}}    %% to be redefined for A&A, small caps
\def\AlI{\mbox{Al\,\specchar{i}}}  %% \def, not \newcommand, for overwrites 
\def\BI{\mbox{B\,\specchar{i}}}    %% use \AlI\ for space behind it
\def\BII{\mbox{B\,\specchar{ii}}}  
\def\BaI{\mbox{Ba\,\specchar{i}}}  
\def\BaII{\mbox{Ba\,\specchar{ii}}} 
\def\CI{\mbox{C\,\specchar{i}}} 
\def\CII{\mbox{C\,\specchar{ii}}} 
\def\CIII{\mbox{C\,\specchar{iii}}} 
\def\CIV{\mbox{C\,\specchar{iv}}} 
\def\CaI{\mbox{Ca\,\specchar{i}}} 
\def\CaII{\mbox{Ca\,\specchar{ii}}} 
\def\CaIII{\mbox{Ca\,\specchar{iii}}} 
\def\CoI{\mbox{Co\,\specchar{i}}} 
\def\CrI{\mbox{Cr\,\specchar{i}}} 
\def\CriI{\mbox{Cr\,\specchar{ii}}} 
\def\CsI{\mbox{Cs\,\specchar{i}}} 
\def\CsII{\mbox{Cs\,\specchar{ii}}} 
\def\CuI{\mbox{Cu\,\specchar{i}}} 
\def\FeI{\mbox{Fe\,\specchar{i}}} 
\def\FeII{\mbox{Fe\,\specchar{ii}}} 
\def\FeIX{\mbox{Fe\,\specchar{ix}}}
\def\FeX{\mbox{Fe\,\specchar{x}}}
\def\FeXIV{\mbox{Fe\,\specchar{xiv}}}
\def\FeXVI{\mbox{Fe\,\specchar{xvi}}}
\def\FrI{\mbox{Fr\,\specchar{i}}}
\def\HI{\mbox{H\,\specchar{i}}} 
\def\HII{\mbox{H\,\specchar{ii}}} 
\def\Hmin{\hbox{\rmH$^{^{_{\scriptstyle -}}}$}}      %% H^min, elegant
\def\Hemin{\hbox{{\rm He}$^{^{_{\scriptstyle -}}}$}} %% He^min, idem
\def\HeI{\mbox{He\,\specchar{i}}} 
\def\HeII{\mbox{He\,\specchar{ii}}} 
\def\HeIII{\mbox{He\,\specchar{iii}}} 
\def\KI{\mbox{K\,\specchar{i}}} 
\def\KII{\mbox{K\,\specchar{ii}}} 
\def\KIII{\mbox{K\,\specchar{iii}}} 
\def\LiI{\mbox{Li\,\specchar{i}}} 
\def\LiII{\mbox{Li\,\specchar{ii}}} 
\def\LiIII{\mbox{Li\,\specchar{iii}}} 
\def\MgI{\mbox{Mg\,\specchar{i}}} 
\def\MgII{\mbox{Mg\,\specchar{ii}}} 
\def\MgIII{\mbox{Mg\,\specchar{iii}}} 
\def\MnI{\mbox{Mn\,\specchar{i}}} 
\def\NI{\mbox{N\,\specchar{i}}}
\def\NaI{\mbox{Na\,\specchar{i}}}
\def\NaII{\mbox{Na\,\specchar{ii}}}
\def\NaIII{\mbox{Na\,\specchar{iii}}} 
\def\NiI{\mbox{Ni\,\specchar{i}}} 
\def\NiII{\mbox{Ni\,\specchar{ii}}}
\def\NiIII{\mbox{Ni\,\specchar{iii}}} 
\def\OI{\mbox{O\,\specchar{i}}} 
\def\OVI{\mbox{O\,\specchar{vi}}}
\def\RbI{\mbox{Rb\,\specchar{i}}} 
\def\RrI{\mbox{Rr\,\specchar{i}}}      %% Robruttenium I
\def\RrII{\mbox{Rr\,\specchar{ii}}}    %% Robruttenium II
\def\RrIII{\mbox{Rr\,\specchar{iii}}}  %% Robruttenium III
\def\SII{\mbox{S\,\specchar{ii}}} 
\def\SiI{\mbox{Si\,\specchar{i}}} 
\def\SiII{\mbox{Si\,\specchar{ii}}} 
\def\SrI{\mbox{Sr\,\specchar{i}}}
\def\SrII{\mbox{Sr\,\specchar{ii}}}
\def\TiI{\mbox{Ti\,\specchar{i}}} 
\def\TiII{\mbox{Ti\,\specchar{ii}}} 
\def\TiIII{\mbox{Ti\,\specchar{iii}}} 
\def\TiIV{\mbox{Ti\,\specchar{iv}}} 
\def\VI{\mbox{V\,\specchar{i}}} 
\def\HtwoO{\mbox{H$_2$O}}        %% H2O
\def\Otwo{\mbox{O$_2$}}          %% O2

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LINES

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Ba II
\def\BaIIres{\mbox{Ba\,\specchar{ii} 4554\,\AA}} %% yak, no numbers

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% hydrogen
\def\Halpha{\mbox{H\hspace{0.1ex}$\alpha$}} %% \Halpha\ for space behind it
\def\Ha{\mbox{H\hspace{0.2ex}$\alpha$}}
\def\Hbeta{\mbox{H\hspace{0.2ex}$\beta$}}
\def\Hgamma{\mbox{H\hspace{0.2ex}$\gamma$}}
\def\Hdelta{\mbox{H\hspace{0.2ex}$\delta$}}
\def\Hepsilon{\mbox{H\hspace{0.2ex}$\epsilon$}}
\def\Hzeta{\mbox{H\hspace{0.2ex}$\zeta$}}
\def\Lyalpha{\mbox{Ly$\hspace{0.2ex}\alpha$}}
\def\Lybeta{\mbox{Ly$\hspace{0.2ex}\beta$}}
\def\Lygamma{\mbox{Ly$\hspace{0.2ex}\gamma$}}
\def\Lycont{\mbox{Ly\hspace{0.2ex}{\small cont}}}
\def\Baalpha{\mbox{Ba$\hspace{0.2ex}\alpha$}}
\def\Babeta{\mbox{Ba$\hspace{0.2ex}\beta$}}
\def\Bacont{\mbox{Ba\hspace{0.2ex}{\small cont}}}
\def\Paalpha{\mbox{Pa$\hspace{0.2ex}\alpha$}}
\def\Bralpha{\mbox{Br$\hspace{0.2ex}\alpha$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Na D
\def\NaD{\mbox{Na\,\specchar{i}\,D}}    %% use \NaD\ for space behind it
\def\NaDone{\mbox{Na\,\specchar{i}\,\,D$_1$}}
\def\NaDtwo{\mbox{Na\,\specchar{i}\,\,D$_2$}}
\def\NaID{\mbox{Na\,\specchar{i}\,\,D}}
\def\NaIDone{\mbox{Na\,\specchar{i}\,\,D$_1$}}
\def\NaIDtwo{\mbox{Na\,\specchar{i}\,\,D$_2$}}
\def\Done{\mbox{D$_1$}}
\def\Dtwo{\mbox{D$_2$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Mg b
\def\Mgbone{\mbox{Mg\,\specchar{i}\,b$_1$}}
\def\Mgbtwo{\mbox{Mg\,\specchar{i}\,b$_2$}}
\def\Mgbthree{\mbox{Mg\,\specchar{i}\,b$_3$}}
\def\MgIb{\mbox{Mg\,\specchar{i}\,b}}
\def\MgIbone{\mbox{Mg\,\specchar{i}\,b$_1$}}
\def\MgIbtwo{\mbox{Mg\,\specchar{i}\,b$_2$}}
\def\MgIbthree{\mbox{Mg\,\specchar{i}\,b$_3$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Ca II H & K 
\def\CaIIK{\mbox{Ca\,\specchar{ii}\,\,K}}       %% use \CaIIK\ for space
\def\CaIIH{\mbox{Ca\,\specchar{ii}\,\,H}}
\def\CaIIHK{\mbox{Ca\,\specchar{ii}\,\,H\,\&\,K}}
\def\HK{\mbox{H\,\&\,K}}
\def\Kthree{\mbox{K$_3$}}      %% numbers not permitted, dammit
\def\Hthree{\mbox{H$_3$}}
\def\Ktwo{\mbox{K$_2$}}
\def\Htwo{\mbox{H$_2$}}
\def\Kone{\mbox{K$_1$}}     
\def\Hone{\mbox{H$_1$}}     
\def\KtwoV{\mbox{K$_{2V}$}}
\def\KtwoR{\mbox{K$_{2R}$}}
\def\KoneV{\mbox{K$_{1V}$}}
\def\KoneR{\mbox{K$_{1R}$}}
\def\HtwoV{\mbox{H$_{2V}$}}
\def\HtwoR{\mbox{H$_{2R}$}}
\def\HoneV{\mbox{H$_{1V}$}}
\def\HoneR{\mbox{H$_{1R}$}}
\def\Kg{{\KtwoV\ grain}}
\def\Kgs{{\KtwoV\ grains}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Mg II h & k 

\def\MgIIk{\mbox{Mg\,\specchar{ii}\,\,k}}
\def\MgIIh{\mbox{Mg\,\specchar{ii}\,\,h}}
\def\MgIIhk{\mbox{Mg\,\specchar{ii}\,\,h\,\&\,k}}
\def\hk{\mbox{h\,\&\,k}}
\def\kthree{\mbox{k$_3$}}    
\def\hthree{\mbox{h$_3$}}
\def\ktwo{\mbox{k$_2$}}
\def\htwo{\mbox{h$_2$}}
\def\kone{\mbox{k$_1$}}     
\def\hone{\mbox{h$_1$}}     
\def\ktwoV{\mbox{k$_{2V}$}}
\def\ktwoR{\mbox{k$_{2R}$}}
\def\koneV{\mbox{k$_{1V}$}}
\def\koneR{\mbox{k$_{1R}$}}
\def\htwoV{\mbox{h$_{2V}$}}
\def\htwoR{\mbox{h$_{2R}$}}
\def\honeV{\mbox{h$_{1V}$}}
\def\honeR{\mbox{h$_{1R}$}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ATOMIC LEVEL
%% use:    \level 3s3p 3Pe
%%         \level 3s$^2$ {1,3}P{e,o}
%%         \level {} 3Ge
%%
\def\level #1 #2#3#4{$#1 \: ^{#2} \mbox{#3} ^{#4}$}   

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STAR NAME
\newcommand{\starname}[2]{${#1}$\,{\rm {#2}}}  %% \starname{\alpha}{Cen~A} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ROMAN CHARACTERS FOR MATH 
\def\rma{{\rm a}} \def\rmA{{\rm A}}             %% without space 
\def\rmb{{\rm b}} \def\rmB{{\rm B}}             %% use for indices etc. 
\def\rmc{{\rm c}} \def\rmC{{\rm C}} 
\def\rmd{{\rm d}} \def\rmD{{\rm D}} 
\def\rme{{\rm e}} \def\rmE{{\rm E}} 
\def\rmf{{\rm f}} \def\rmF{{\rm F}} 
\def\rmg{{\rm g}} \def\rmG{{\rm G}} 
\def\rmh{{\rm h}} \def\rmH{{\rm H}} 
\def\rmi{{\rm i}} \def\rmI{{\rm I}} 
\def\rmj{{\rm j}} \def\rmJ{{\rm J}} 
\def\rmk{{\rm k}} \def\rmK{{\rm K}} 
\def\rml{{\rm l}} \def\rmL{{\rm L}} 
\def\rmm{{\rm m}} \def\rmM{{\rm M}} 
\def\rmn{{\rm n}} \def\rmN{{\rm N}} 
\def\rmo{{\rm o}} \def\rmO{{\rm O}} 
\def\rmp{{\rm p}} \def\rmP{{\rm P}} 
\def\rmq{{\rm q}} \def\rmQ{{\rm Q}} 
\def\rmr{{\rm r}} \def\rmR{{\rm R}} 
\def\rms{{\rm s}} \def\rmS{{\rm S}} 
\def\rmt{{\rm t}} \def\rmT{{\rm T}} 
\def\rmu{{\rm u}} \def\rmU{{\rm U}} 
\def\rmv{{\rm v}} \def\rmV{{\rm V}} 
\def\rmw{{\rm w}} \def\rmW{{\rm W}} 
\def\rmx{{\rm x}} \def\rmX{{\rm X}} 
\def\rmy{{\rm y}} \def\rmY{{\rm Y}} 
\def\rmz{{\rm z}} \def\rmZ{{\rm Z}} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% UNITS
\def\deg{\hbox{$^\circ$}}       %% \def for overwriting, \box for math
\def\degree{\hbox{$^\circ$}}
\def\degrees{\hbox{$^\circ$}}
\def\arcmin{\hbox{$^\prime$}}
\def\bgmin{\hbox{$^\prime$}}
\def\arcsec{\hbox{$^{\prime\prime}$}}
\def\secarc{\hbox{$^{\prime\prime}$}}
\def\bgsec{\hbox{$^{\prime\prime}$}}
\def\kms{\hbox{km$\;$s$^{-1}$}}
\def\micron{\hbox{$\mu$m}}
\def\kayser{\hbox{$\rm cm^{-1}$}}
\def\Mxcm{\hbox{Mx\,cm$^{-2}$}}    %% no 2, damn tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% VARIA
\def\is{\!=\!}                             %% = in text for tighter spacing
\def\dif{\: {\rm d}}                       %% differential d with space
\def\ep{\:{\rm e}^}                        %% e^ with space and roman e
\def\dash{\hbox{$\,-\,$}}                  %% math-like hyphen

\def\lambdop{\hbox{$\bf \Lambda$}}         %% plain Lambda operator

\def\gf{\mbox{$g \! f$}}                   %% \gf\ for space behind it

\def\ko{($k, \omega$)}                     %% k - omega 
\def\komega{($k, \omega$)}                 %% k - omega 
\def\kf{($k_h,f$)}                         %% f - k_h
\def\VminI{\hbox{$V\!\!-\!\!I$}}           %% V-I
\def\IminI{\hbox{$I\!\!-\!\!I$}}           %% I-I
\def\VminV{\hbox{$V\!\!-\!\!V$}}           %% V-V
\def\Xt{\hbox{$X\!\!-\!t$}}                %% X-t
\def\={\hbox{$\!=\!$}}                     %% less space around =

\def\sun{\hbox{$\odot$}}                   %% Sun symbol
\def\earth{\hbox{$\oplus$}}                %% Earth symbol

\def\BminV{\hbox{$B\!\!-\!\!V$}}           %% B-V
\def\VminIk{\hbox{$(V\!\!-\!\!I)_K$}}      %% V-I_K
\def\Teff{\hbox{$T_{\rm eff}$}}            %% T_eff

\def\Bapp{\hbox{$B_{\rm app}$}}              %% apparent flux density
\def\Basp{\hbox{$B_{\rm app}^{\rm ASP}$}}    %% apparent flux density ASP
\def\Bbbso{\hbox{$B_{\rm app}^{\rm BBSO}$}}  %% idem BBSO
\def\Bkpno{\hbox{$B_{\rm app}^{\rm KPNO}$}}  %% idem KPNO

\def\dotpp{DOT$^{\mbox{\small \boldmath ++}}$} %% DOT++ proposal (alas)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% stacked math symbols
%% macro by Louis Strous, after char.mac Skumanich Soesterberg 
%% usage: \mathstacksym\newsymbol{upper_symbol}{lower_symbol}
%%                               {upper_height}{lower_depth}
\def\mathstacksym#1#2#3#4#5{\def#1{\mathrel{\hbox to 0pt{\lower 
    #5\hbox{#3}\hss} \raise #4\hbox{#2}}}}

\mathstacksym\lta{$<$}{$\sim$}{1.5pt}{3.5pt} % less than approximately
\mathstacksym\gta{$>$}{$\sim$}{1.5pt}{3.5pt} % greater than approximately
\mathstacksym\lrarrow{$\leftarrow$}{$\rightarrow$}{2pt}{1pt} % equilibrium
\mathstacksym\lessgreat{$>$}{$<$}{3pt}{3pt} %% less or greater

%%%%%%%%%%%%%%%%%%%%  END OF FILE RRMACROS.TEX  %%%%%%%%%%%%%%%%%%%%%%%%%%%


